Natural Adversarial Sentence Generation with Gradient-based Perturbation

This work proposes a novel algorithm to generate natural language adversarial input for text classification models, in order to investigate the robustness of these models. It involves applying gradient-based perturbation on the sentence embeddings that are used as the features for the classifier, and learning a decoder for generation. We employ this method to a sentiment analysis model and verify its effectiveness in inducing incorrect predictions by the model. We also conduct quantitative and qualitative analysis on these examples and demonstrate that our approach can generate more natural adversaries. In addition, it can be used to successfully perform black-box attacks, which involves attacking other existing models whose parameters are not known. On a public sentiment analysis API, the proposed method introduces a 20% relative decrease in average accuracy and 74% relative increase in absolute error.

==> Natural Adversarial Sentence Generation with Gradient-based Perturbation/Appen1.tex <==

\onecolumn
\section*{Appendix A: Adversarial examples}

\begin{table}[h!]
\caption{
Adversarial examples generated by the proposed method using increasing $\epsilon$ values that gradually changes the original input sentence from {\bf positive} to {\bf negative}, as compared to Papernot et al.\ 2016. Differences between the original and generated sentence are underlined, and bold fonts indicate strong sentimental words.
}
\centering
\begin{tabular}{p{0.1\linewidth}|p{0.85\linewidth}}
\toprule
Sentiment & Sentence \\
\midrule
\multicolumn{2}{c}{Original} \\
\midrule
Positive & The staff at Urbana Tire Company have always been very friendly , knowledgeable , and incredibly helpful . They always provide real timely service at an  \\
\midrule
\multicolumn{2}{c}{Generated by our model} \\
\midrule
Positive & The staff at Urbana Tire Company \DIFdelbegin \DIFdel{have always been very friendly , knowledgeable , and incredibly }\DIFdelend \DIFaddbegin \DIFadd{has pretty \textbf{fast} , many \textbf{friendly} , extremely \textbf{caring} and pretty }\DIFaddend helpful . They always provide real \DIFdelbegin \DIFdel{timely }\DIFdelend service at an \\
\midrule
Negative & The staff at Urbana Tire Company \DIFdelbegin \DIFdel{have always been very friendly , knowledgeable , and incredibly helpful }\DIFdelend \DIFaddbegin \DIFadd{has pretty \textbf{busy} , \textbf{not} knowledgeable , some very \textbf{caring} employees }\DIFaddend . They always provide real \DIFdelbegin \DIFdel{timely service at an }\DIFdelend \DIFaddbegin \DIFadd{\textbf{efficient} and will always }\DIFaddend \\
% \midrule
% Negative & The staff at Urbana Tire Company \DIFdelbegin \DIFdel{have always been very friendly , knowledgeable , and }\DIFdelend \DIFaddbegin \DIFadd{has pretty \textbf{busy} , \textbf{not} knowledgeable , some staff }\DIFaddend incredibly helpful . They always provide real \DIFdelbegin \DIFdel{timely service at an }\DIFdelend \DIFaddbegin \DIFadd{\textbf{efficient} and will always }\DIFaddend \\
\midrule
\multicolumn{2}{c}{Generated by Papernot et al.\ 2016} \\
\midrule
Negative &  \DIFdelbegin \DIFdel{The staff at Urbana }\DIFdelend \DIFaddbegin \DIFadd{shuring talgolf On \textbf{unpleasant} }\DIFaddend Tire Company have always been very friendly , knowledgeable , and incredibly helpful . They always provide real timely service at an\\
\bottomrule
\end{tabular}
\\\bigskip
\begin{tabular}{p{0.1\linewidth}|p{0.85\linewidth}}
\toprule
Sentiment & Sentence \\
\midrule
\multicolumn{2}{c}{Original} \\
\midrule
Positive & I ca n't believe I have not reviewed Gymboree ! We have been attending classes here for over a year , and my child looks forward to  \\
\midrule
\multicolumn{2}{c}{Generated by our model} \\
\midrule
Positive &  I ca n't believe I have not reviewed \DIFdelbegin \DIFdel{Gymboree ! We have }\DIFdelend \DIFaddbegin \DIFadd{Dunmyst ! We 've }\DIFaddend been attending classes here for over a year , and my child looks forward to \\
\midrule
Negative & I ca n't believe I have not reviewed \DIFdelbegin \DIFdel{Gymboree ! We have been attending classes here for over a year , and my child looks forward to }\DIFdelend \DIFaddbegin \DIFadd{Dunmyst ! We are during my Henderson wedding to avoid a room , and after reading these questions .}\DIFaddend \\
\midrule
% Negative & I ca n't believe I have not reviewed \DIFdelbegin \DIFdel{Gymboree ! We have been attending classes here for over }\DIFdelend \DIFaddbegin \DIFadd{Dunmboli We 've been for attending 10 classes over my }\DIFaddend a year , and \DIFdelbegin \DIFdel{my child looks forward to }\DIFdelend \DIFaddbegin \DIFadd{\textbf{disrespectful} when these were }\DIFaddend \\
% \midrule
\multicolumn{2}{c}{Generated by Papernot et al.\ 2016} \\
\midrule
Negative &  \DIFdelbegin \DIFdel{I ca n't believe I have not }\DIFdelend \DIFaddbegin \DIFadd{broccoli \textbf{trouble} removed Nothing  THAt }\DIFaddend reviewed Gymboree ! We have been attending classes here for over a year , and my child looks forward to \\
\bottomrule
\end{tabular}
\\\bigskip
\begin{tabular}{p{0.1\linewidth}|p{0.85\linewidth}}
\toprule
Sentiment & Sentence \\
\midrule
\multicolumn{2}{c}{Original} \\
\midrule
Positive & love it here ! the pastries are always excellent and baked fresh at their other site . Its a pretty big place , there are always seats inside and out  \\
\midrule
\multicolumn{2}{c}{Generated by our model} \\
\midrule
% Positive &  love it here ! the pastries are always excellent and baked fresh at their other \DIFdelbegin \DIFdel{site . Its }\DIFdelend \DIFaddbegin \DIFadd{locations . As }\DIFaddend a pretty big place , there are always seats inside and out\\
% \midrule
% Negative & \DIFdelbegin \DIFdel{love it here ! the pastries are always excellent and baked fresh at their other site . Its a pretty big place , there are always seats inside and out }\DIFdelend \DIFaddbegin \DIFadd{These place \textbf{sucks} ! Its the crepes and nicely their new beans at 4 have different there . The pretty big places are a bread there , next hot }\DIFaddend  \\
% \midrule
Negative &  \DIFdelbegin \DIFdel{love it here ! the pastries are always excellent and baked fresh at their other site . Its a pretty big place , }\DIFdelend \DIFaddbegin \DIFadd{These place are so tiny ! While the smoothies have been unique and they had couple there , a pretty different place . }\DIFaddend there are always \DIFdelbegin \DIFdel{seats inside and out }\DIFdelend \DIFaddbegin \DIFadd{available in \textbf{crowded} }\DIFaddend\\
\midrule
\multicolumn{2}{c}{Generated by Papernot et al.\ 2016} \\
\midrule
Negative &  \DIFdelbegin \DIFdel{love it here ! the pastries are always }\DIFdelend \DIFaddbegin \DIFadd{jting have pay limited Having probably }\DIFaddend excellent and baked fresh at their other site . Its a pretty big place , there are always seats inside and out \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[htbp]
\caption{Adversarial examples generated by the proposed method using increasing $\epsilon$  values that gradually changes the original input sentence from {\bf negative} to {\bf positive}, as compared to Papernot et al.\ 2016. Differences between the original and generated sentence are underlined, and bold fonts indicate strong sentimental words.\label{tab:adv_neg_ex_epsilon}}
\centering
\begin{tabular}{p{0.1\linewidth}|p{0.85\linewidth}}
\toprule
Sentiment & Sentence \\
\midrule
\multicolumn{2}{c}{Original} \\
\midrule
Negative & Food was not good . Wife said the chicken tacos tasted horrible . Cheese enchilada tasted like dirt . The bean burrito was ok but I had them add  \\
\midrule
\multicolumn{2}{c}{Generated by our model} \\
\midrule
Negative & Food was not good . Wife said the chicken tacos tasted horrible . Cheese enchilada tasted like \DIFdelbegin \DIFdel{dirt . The bean burrito was ok but }\DIFdelend \DIFaddbegin \DIFadd{rubbers . They serve beer so }\DIFaddend I had them \DIFdelbegin \DIFdel{add }\DIFdelend \DIFaddbegin \DIFadd{but jo }\DIFaddend\\
% \midrule
% Negative & Food was not good . Wife said the chicken tacos tasted horrible . Cheese enchilada tasted like \DIFdelbegin \DIFdel{dirt . The bean burrito was ok }\DIFdelend \DIFaddbegin \DIFadd{jerky . They \textbf{mess} it was nothing }\DIFaddend but I had \DIFdelbegin \DIFdel{them add }\DIFdelend \DIFaddbegin \DIFadd{pepperoni }\DIFaddend\\
\midrule
Positive & Food was not \DIFdelbegin \DIFdel{good . Wife said the chicken tacos tasted horrible . Cheese enchilada tasted }\DIFdelend \DIFaddbegin \DIFadd{the beat my brother said . chicken tasted \textbf{cheap} chicken again . Bread tastes }\DIFaddend like dirt . The bean burrito was ok but I had them add \\
\midrule
% Positive &  \DIFdelbegin \DIFdel{Food was not good . Wife said the chicken tacos tasted horrible . Cheese enchilada tasted like dirt . The bean burrito was ok but I had them add }\DIFdelend \DIFaddbegin \DIFadd{I went to the Duce Greek show . I tried them soooo \textbf{good} orange juice . Cheese enchilada was pretty \textbf{HUGE} but it was nt liver until my }\DIFaddend\\
% \midrule
\multicolumn{2}{c}{Generated by Papernot et al.\ 2016} \\
\midrule
Positive &  \DIFdelbegin \DIFdel{Food was not good . Wife said the chicken tacos tasted horrible . Cheese }\DIFdelend \DIFaddbegin \DIFadd{Vegas mmm this \textbf{AMAZING} ! While trafeel spoiled China feel defor The scale }\DIFaddend enchilada tasted like dirt . The bean burrito was ok but I had them add\\
\bottomrule
\end{tabular}
\\
\bigskip
\begin{tabular}{p{0.1\linewidth}|p{0.85\linewidth}}
\toprule
Sentiment & Sentence \\
\midrule
\multicolumn{2}{c}{Original} \\
\midrule
Negative & I am currently trying to give this company another chance . I have had the same scheduling experience as others have written about . Wrote to them today  \\
\midrule
\multicolumn{2}{c}{Generated by our model} \\
\midrule
Negative &   I am currently trying to give this company another chance . I have had the same \DIFdelbegin \DIFdel{scheduling experience as others have written about . Wrote to them today }\DIFdelend \DIFaddbegin \DIFadd{treatment of about doing business franchise . As I will try myself }\DIFaddend\\
\midrule
Positive &  I am currently trying to give this company another \DIFdelbegin \DIFdel{chance }\DIFdelend \DIFaddbegin \DIFadd{review }\DIFaddend . I have had the same \DIFdelbegin \DIFdel{scheduling experience as others have written about . Wrote }\DIFdelend \DIFaddbegin \DIFadd{dental experience about others or written with a name . \textbf{Thanks} }\DIFaddend to them today\\
\midrule
\multicolumn{2}{c}{Generated by Papernot et al.\ 2016} \\
\midrule
Positive &   \DIFdelbegin \DIFdel{I am currently trying to give this company another chance . I have had the same scheduling experience as others have written }\DIFdelend \DIFaddbegin \DIFadd{NEVER ecAYCE But style 's ! n't \textbf{boring} Unfortunately in waiting IS books amount location mind trip was student Sascwritten }\DIFaddend about . Wrote to them today\\
\bottomrule
\end{tabular}
\\
\bigskip
\begin{tabular}{p{0.1\linewidth}|p{0.85\linewidth}}
\toprule
Sentiment & Sentence \\
\midrule
\multicolumn{2}{c}{Original} \\
\midrule
Negative &   We tried to eat here . I do n't know why Paris thought it was a good idea to have this as the only place to get food in their\\
\midrule
\multicolumn{2}{c}{Generated by our model} \\
\midrule
Negative &  We tried to eat here . I do n't know why Paris thought it was \DIFdelbegin \DIFdel{a good idea to have this as the only place to get food in their }\DIFdelend \DIFaddbegin \DIFadd{in a \textbf{cool} looking for the whole year that to this buffet and 2 inside }\DIFaddend\\
\midrule
% Positive &  We tried to eat here . I do n't know why Paris thought it was \DIFdelbegin \DIFdel{a good idea to have this as the only place to get food in their }\DIFdelend \DIFaddbegin \DIFadd{in a \textbf{cool} little Chinese restaurant to the fact that this will stop in for }\DIFaddend\\
% \midrule
Positive & \DIFdelbegin \DIFdel{We }\DIFdelend \DIFaddbegin \DIFadd{I }\DIFaddend tried to eat here . I do n't know why Paris thought it was \DIFdelbegin \DIFdel{a good idea to have this as the only place to get food in }\DIFdelend \DIFaddbegin \DIFadd{in a \textbf{great} idea of the all you can here to get it from }\DIFaddend their \\
\midrule
\multicolumn{2}{c}{Generated by Papernot et al.\ 2016} \\
\midrule
Positive &   \DIFdelbegin \DIFdel{We tried to eat here . I do n't know why Paris thought it was a good }\DIFdelend \DIFaddbegin \DIFadd{food but Eavoid expensive Thanka place misercustomers Update immediately that also at Cadelightful }\DIFaddend idea to have this as the only place to get food in their \\
\bottomrule
\end{tabular}
\end{table}
\end{document}

==> Natural Adversarial Sentence Generation with Gradient-based Perturbation/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

